RasterNet: Modeling Free-Flow Speed using LiDAR and Overhead Imagery

Roadway free-flow speed captures the typical vehicle speed in low traffic conditions. Modeling free-flow speed is an important problem in transportation engineering with applications to a variety of design, operation, planning, and policy decisions of highway systems. Unfortunately, collecting large-scale historical traffic speed data is expensive and time consuming. Traditional approaches for estimating free-flow speed use geometric properties of the underlying road segment, such as grade, curvature, lane width, lateral clearance and access point density, but for many roads such features are unavailable. We propose a fully automated approach, RasterNet, for estimating free-flow speed without the need for explicit geometric features. RasterNet is a neural network that fuses large-scale overhead imagery and aerial LiDAR point clouds using a geospatially consistent raster structure. To support training and evaluation, we introduce a novel dataset combining free-flow speeds of road segments, overhead imagery, and LiDAR point clouds across the state of Kentucky. Our method achieves state-of-the-art results on a benchmark dataset.

==> attic.tex <==
\section{Dataset}

\begin{figure}
\centering
    \begin{subfigure}{.49\linewidth}
        \includegraphics[width=\linewidth]{images/dataset_examples/urban_sat.pdf}
        \caption{Urban Satellite Image}
    \end{subfigure}
    \begin{subfigure}{.49\linewidth}
        \includegraphics[width=\linewidth]{images/dataset_examples/rural_sat.pdf}
        \caption{Rural Satellite Image}
    \end{subfigure}
    
    \begin{subfigure}{\linewidth}
        \includegraphics[trim=17px 7px 6px 0px, clip, width=\linewidth]{images/dataset_examples/urban_side.pdf}
        \caption{Urban Point Cloud}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
        \includegraphics[trim=10px 10px 10px 70px, clip, width=\linewidth]{images/dataset_examples/rural_side2.pdf}
        \caption{Rural Point Cloud}
    \end{subfigure}
    \caption{Examples of our multi-modal dataset. The same urban scene is depicted in satellite image (a) and point cloud (c), and the rural scene in overhead image (b) is the same scene shown in point cloud (d). Point cloud coloring reflects the relative grayscale light intensities.}
    \label{fig:dataset_ex}
\end{figure}

We present a new point cloud dataset for free-flow speed estimation of road segments. Our dataset contains 3D point clouds of road segments that geospatially correspond with georeferenced free-flow speed labels. The dataset is representative of rural, urban, highway and arterial roads across the state of Kentucky. Roads range in structure from one-way dirt/gravel roads to multi-lane highways. Change in elevation, road curvature, lane delineation markings, lane width, proximity to neighboring structures, and other high level spatial features can be uniquely extracted from point clouds but not from overhead images. Augmenting the existing Song et al.~\cite{song2019remote} satellite imagery dataset with our dataset, we enable data fusion and standalone approaches to train for the task of free-flow speed estimation. Point cloud representations of road segments can be combined with overhead imagery by coordinating data representations using geospatial coordinates. We begin by revisiting the Song et al.~\cite{song2019remote} satellite imagery and free-flow speed data set, follow by describing the construction of a LiDAR point cloud dataset, and then characterize the raster method of fusing point clouds with overhead images.

\subsection{Free-Flow Speed and Satellite Imagery}

Georeferenced free-flow speed labels were treated as a set of reference points with which we could bind sensory information. The speed data expressed free-flow speed of a vehicle on a road segment as the speed at which an operator would drive in uncongested traffic on non-holiday weekdays between the hours of 9am and 3pm. The Kentucky Transportation Center~\cite{chen2015analysis} aggregated HERE technologies speed data across uncongested periods to extract and average free-flow speeds of road segments and their corresponding geospatial coordinates. The Song et al.~\cite{song2019remote} dataset used these geospatial coordinates corresponding to the free-flow speed labels to select overhead images centered on the given road segment. The 1m ground-sample distance (GSD) satellite imagery, sourced from the National Agriculture Imagery Program (NAIP), was used to depict $200 \times 200m^2$ roadway scenes. Each image was resized to 224x224 pixels and rotated to ensure roads were aligned with an upward direction of travel. We incorporated satellite imagery into our multi-model dataset to leverage its consistent and structured visual representation of roadway scenes.

\subsection{Airborne LiDAR}
Construction of the point cloud dataset consisted of LiDAR tile selection and point cloud sampling. We aggregated LiDAR data from the Kentucky Division of Geographic Information's KyFromAbove~\cite{kyfromabove} program, which collected aerial LiDAR data over the state of Kentucky USA. The LiDAR data was stored as 31,135 tiles; each of which corresponds to a spatial region of Kentucky. We used an R-tree of the LiDAR tile geospatial locations to match each speed label's coordinate with the tile that contained the label's location. For each selected tile points were randomly sampled read into a k-d tree for fast nearest neighbor search. Point clouds were then sampled by constructing a $200 \times 200m^2$ bounding box centered on the target label location, and then 80 linearly spaced points were selected for each row and column of an 80x80 grid. Each given tile's k-d tree was then used to find the nearest point to each of the sampling grid's point locations. The resulting collection of 6,400 sub-sampled points expressed the spatial features of a given roadway scene.

\subsection{Data Fusion}

An inherent challenge of training deep learning models on point clouds is their lack of fixed and consistent structure. We propose a structural tool, a raster center grid, to impose consistent structure on point cloud features. Structurally consistent point clouds can then be paired with image features in a geospatially consistent manner. As Figure~\ref{fig:raster_pairing} illustrates, each raster center (red dots) binds local neighborhoods of point cloud features to a fixed location in a 7x7 grid, similar to how convolutional neural network's (CNN) group image features. The raster center point grid was generated by constructing a $200 \times 200m^2$ bounding box centered on the target label's geospatial location. Within the bounding box a 7x7 linearly spaced grid was inscribed, and center point of each grid cell was extracted and stored. Integrating the raster center grid into the point cloud dataset enables models to incorporate both point cloud and image features.

%The raster center grid binds local neighborhoods of point cloud features to fixed 7x7 grid, similar to how convolutional neural network's group image features. Each raster cell center (red dots) corresponds to a local point cloud neighborhood of features that is spatially consistent with a region depicted in paired imagery, as shown on the left in Figure~\ref{fig:raster_pairing}.
%The 3D road segment point cloud illustrates the impact the height dimension can have on describing a scene. 

 An overview of the dataset is shown in Figure~\ref{fig:dataset_ex}. The urban road segment depicted in (a) corresponds to the point cloud (c) of the same road segment. The point cloud height features are illustrated by the dark blue low elevation roadways in stark contrast with the red roof tops of sky scrapers (top right). Similarly, the rural road segment point cloud (d) shows the dynamic topography of landscapes neighboring roads not present in the corresponding satellite image (b). Altogether, this dataset allows image-only, point cloud-only, and hybrid image and point cloud models to be trained and evaluated.


